PanoSLAM: Panoptic 3D Scene Reconstruction via Gaussian SLAM

Understanding geometric, semantic, and instance information in 3D scenes from sequential video data is essential for applications in robotics and augmented reality. However, existing Simultaneous Localization and Mapping (SLAM) methods generally focus on either geometric or semantic reconstruction. In this paper, we introduce PanoSLAM, the first SLAM system to integrate geometric reconstruction, 3D semantic segmentation, and 3D instance segmentation within a unified framework. Our approach builds upon 3D Gaussian Splatting, modified with several critical components to enable efficient rendering of depth, color, semantic, and instance information from arbitrary viewpoints. To achieve panoptic 3D scene reconstruction from sequential RGB-D videos, we propose an online Spatial-Temporal Lifting (STL) module that transfers 2D panoptic predictions from vision models into 3D Gaussian representations. This STL module addresses the challenges of label noise and inconsistencies in 2D predictions by refining the pseudo labels across multi-view inputs, creating a coherent 3D representation that enhances segmentation accuracy. Our experiments show that PanoSLAM outperforms recent semantic SLAM methods in both mapping and tracking accuracy. For the first time, it achieves panoptic 3D reconstruction of open-world environments directly from the RGB-D video. (https://github.com/runnanchen/PanoSLAM)

==> sections/method_back.tex <==
Current semantic SLAM methods fails to capture both instance and semantic information of a scene, known as panoptic information. In this section we present a new method, called \textit{PanoSLAM}, that efficiently reconstructs 3D panoptic semantic maps from unlabeled RGBD videos. Essentially, PanoSLAM transfers the knowledge of a 2D vision model into a real-time SLAM system. Specifically, we enhance a real-time Gaussian-based SLAM with the capability to render panoptic information through critical modifications to the Gaussian Splatting-based SLAM. Furthermore, we  develop a new Spatial-temporally Lifting module to learn with noisy labels. In the following we will begin with preliminaries of the Gaussian-based SLAM system, and then explain our modifications to the system and present our Spatial-Temporally Lifting module.

%\vspace*{-1ex}
\subsection{Preliminaries about Gaussian-based SLAM}
\vspace*{-1ex}
Our system is built on SplaTAM~\cite{keetha2023splatam}, a SOTA dense RGB-D SLAM solution that utilizes 3D Gaussian Splatting. By representing the world as a set of 3D Gaussians that can be transformed into detailed color and depth images, it employs differentiable rendering and gradient-based optimization to simultaneously optimize the camera pose for each frame and a discrete volumetric map of the environment. We begin with a brief overview of 3D Gaussian Splatting and then describe each module of SplaTAM. 
\vspace*{-1ex}
\paragraph{Gaussian Representation.}
SplaTAM simplifies the Gaussian representation by using solely view-independent color and ensuring that the Gaussians are isotropic. This means that each Gaussian is defined by only eight values, including three for its RGB color $\bold c\in \mathbb{R}^3$, three for the center position $\bold u\in \mathbb{R}^3$, one for the radius (i.e. the standard deviation) $r$, and one for the opacity $o$. Each Gaussian has an impact on a point in 3D space $\bold x\in \mathbb{R}^3$ based on the standard (unnormalized) Gaussian equation, weighted by its opacity:
\begin{equation}\label{equ:Gaussian}
f(x)=o\exp \left(-\frac{\parallel \bold x-\bold u\parallel^2}{2r^2}\right),
\end{equation}
\vspace*{-1ex}
\paragraph{Differentiable Rendering via Splatting.}
SplaTAM renders an RGB image by sorting a collection of 3D Gaussians from front to back and then efficiently alpha-compositing the splatted 2D projection of each Gaussian in pixel space. The color of a rendered pixel $P = (u,v)$ can be expressed as:
\begin{equation}\label{equ:Rendering}
C(P)=\sum_{i=1}^{n}c_if_i(P)\prod_{j=1}^{i-1}(1-f_{i}(P)),
\end{equation}
where $f_i(P)$ is calculated according to Eq. \ref{equ:Gaussian}, using the $\bold u$ and $r$ values of the splatted 2D Gaussians in pixel space: 
\begin{equation}\label{equ:2DGaussian}
\bold u^{2D}=G\frac{E_t \bold u}{d},\;\;\; r^{2D}=\frac{fr}{d},\;\;\; d=(E_t \bold u)_z,
\end{equation}
where the variables $G$, $E_t$, $f$, and $d$ represent the camera intrinsic matrix, extrinsic matrix for the rotation and translation of the camera at frame $t$, focal length (known), and the depth of the $i$-th Gaussian in camera coordinates, respectively.


%\vspace*{-1ex}
\subsection{PanoSLAM}
\vspace*{-1ex}
Built on Gaussian-based SLAM, our PanoSLAM method integrates knowledge from a 2D vision model into the Gaussian SLAM system to efficiently reconstruct 3D panoptic semantic maps from unlabeled RGBD videos. This involves implementing significant modifications to enable Splatting-based SLAM to render panoptic information, such as semantic Gaussian initialization and densification and panoptic segmentation formulation. Additionally, we make use of the 2D vision model's panoptic prediction, including instances and semantic predictions, as pseudo labels to aid in guiding 3D panoptic semantic map reconstruction. However, these pseudo labels are prone to label noise, including inconsistent mask prediction and inconsistent mask class prediction across different views, causing optimization conflicts and corrupting the semantic map reconstruction. To address the impact of noisy pseudo labels, we propose a Spatial-Temporally Lifting module. In the following, we will explain the steps and insights of PanoSLAM.

\vspace*{-1ex}
\paragraph{Semantic Gaussian Representation, Initialization and Densification.}
Unlike SplaTAM where each Gaussian is parameterized by 8 values, PanoSLAM assigns 13 values for each Gaussian for rendering semantic representation as follows: three values for its semantic embedding $\bold s\in \mathbb{R}^3$, one for its semantic radius $\hat{r}$ (i.e., standard deviation), and one for semantic opacity $\hat{o}$, plus the same 8 values used in SplaTAM. Thus, the rendered semantic embedding of pixel $P = (u,v)$ can be represented as:
\begin{equation}\label{equ:Rendering_semantics}
S(P)=\sum_{i=1}^{n}\bold s_i\hat{f}_i(P)\prod_{j=1}^{i-1}(1-\hat{f}_{i}(P)),
\end{equation}
where $\hat{f}_i(P)$ is calculated according to Eq. \ref{equ:Gaussian} and \ref{equ:2DGaussian}, using the $\hat{r}$ and $\hat{o}$ values.

To initialize the Gaussians in the first frame, the camera pose is set to identity. We add a new Gaussian for each pixel, the centre $\bold u$ is the unprojection of the pixel depth, and the radius $r$ and semantic radius $\hat{r}$ are both equal to the one-pixel radius of the 2D image \ie,  $\hat{r}=r=\frac{D_{GT}}{f}$. Besides, the color $\bold c$ and semantic embedding $\bold s$ are both initialized to be the pixel color. The optical opacity $o$ and the semantic $\hat{o}$ are both initialized to be 0.5.

To spawn Gaussians (densification) in the subsequent frames, we add Gaussian kernels at locations where the existing ones do not accurately capture the scene's geometry or semantics. To this end, we create the following densification mask to identify the pixels that require densification.
\begin{equation}\label{equ:densification}
\begin{align}M(P)=(F(P) < 0.5)\; {\rm or} \; (\hat{F}(P) < 0.5) \; {\rm or} \\
\;(L(D(P))>T),
\end{align}
\end{equation}
where $D(P)$ is a differentiable rendered depth:
\begin{equation}\label{equ:depth}
D(P)=\sum_{i=1}^{n}d_if_i(P)\prod_{j=1}^{i-1}(1-f_{i}(P)),
\end{equation}
and $\hat{F}(P)$ is silhouette map to determine visibility, calculated by using $\hat{o}$ and $\hat{r}$. 
\begin{equation}\label{equ:silhouette}
\hat{F}(P)=\sum_{i=1}^{n}\hat{f}_i(P)\prod_{j=1}^{i-1}(1-\hat{f}_{i}(P)),
\end{equation}
$T$ is the threshold of depth error exceeds 50 times the median depth error. The densification mask serves two purposes. It helps identify areas where the map lacks sufficient density ($S < 0.5$) in terms of geometry or semantics and flags instances where the ground-truth depth and the rendered depth do not align. For each pixel flagged by this mask, we introduce a new Gaussian following the same initialization process used in the first frame.

\vspace*{-1ex}
\paragraph{Camera Tracking}
Camera tracking involves estimating the camera pose of the current incoming online RGB-D image in the input stream. The camera pose is initialized for a new timestep through a constant velocity forward projection of the pose parameters in the camera centre + quaternion space:
\begin{equation}\label{equ:camera_pose}
E_{t+1}=E_t+(E_t-E_{t-1}).
\end{equation}
The camera pose $E_t$ is then iteratively refined through gradient-based optimization by differentiably rendering RGB, depth, and silhouette maps and adjusting the camera parameters to minimize the loss, while fixing Gaussian parameters.

\vspace*{-1ex}
\paragraph{Panoptic Segmentation Formulation}
Panoptic segmentation is created by combining semantic and instance segmentation. Drawing inspiration from Maskformer \cite{cheng2021per}, we divide the panoptic segmentation task into two parts: 1) dividing the image into $N$ regions using binary masks; and 2) associating each region with a probability distribution of labeling over $K$ categories. Specifically, we first obtain the region's predictions for each pixel $P = (u,v)$:
\begin{equation}\label{equ:region_prediction}
R(P)=\Gamma(S(P)) \otimes \mathbb{M},
\end{equation}
where $R(P) \in \mathbb{R}^N$ is the predicted distribution over $N$ regions, $\mathbb{M} \in \mathbb{R}^{N \times H}$ are $N$ region embeddings with $H$ dimensions, $\Gamma(\bullet)$ is an MLP decoder that increases the semantic embedding's dimension from 3 to $H$, and $\otimes$ donates the matrix multiplication. We classify $N$ regions into $K$ categories as follows
\begin{equation}\label{equ:region_classfication}
O(\mathbb{M})=\mathbb{M} \otimes \mathbb{C},
\end{equation}
where $\mathbb{C} \in \mathbb{R}^{N \times K}$ is the classifier, and $O(\mathbb{M}) \in \mathbb{R}^K$ donates the predicted distribution over $K$ categories. The definitions above effectively assign a pixel at location $P = (u,v)$ to the $i$-th probability-region and $j$-th probability-category only if the most likely class probability $O^j(\mathbb{M})$ and the region prediction probability $R^i(P)$ are both sufficiently large~\cite{cheng2021per}. Additionally, we eliminate low-confidence predictions before inference and discard predicted segments with significant portions of their binary masks occluded by other predictions. 
\vspace*{-1ex}
\paragraph{Spatial-Temporally Lifting}
Given the absence of ground truth labels, for each image frame of the input video sequences,  we utilize the off-the-shelf 2D vision model to perform panoptic prediction for each pixel $P=(u,v)$, including both instances $\{\hat{R}_t(P)\}_{t=1}^T$ and semantics predictions $\{\hat{O}_t(P)\}_{t=1}^T$. Here, $T$ is the number of time steps (i.e., image frames) to be processed. These predictions are then utilized as the pseudo labels to optimize the panoptic segmentation results from PanoSLAM. However, these predictions usually contain noisy labels that may corrupt the optimization process. 

To address this issue, we unify the panoptic prediction across different time steps over the shared 3D shape through multi-view correspondence. To facilitate this, given two pixels $P^{*1}$ and $P^{*2}$ belonging to different views, if their respective unprojected 3D points $\bold P^{*1}$ and $\bold P^{*2}$ are located in the same local small voxel space, we regard these two pixels as being in correspondence.
Specifically, to efficiently identify corresponding pixels across the $T$ frames, we first re-project the pixel depths of each frame to the world coordinates according to their corresponding camera poses and intrinsic (Eq. \ref{equ:project_3D}). These reprojected 3D points are then fused to form a point cloud. The 3D space occupied by this point cloud is uniformly split into voxels with a specified size $S_n$, and we quantize all these points into the centers of voxels directly, allowing us to quickly obtain the corresponding voxel indices. Finally, the points sharing the same voxel index indicate that they are located in the same local small voxel and inherently should have consistent semantic labels for the corresponding pixels across the $T$ frames. This approach allows us to efficiently determine the correspondence of pixels and unify the semantic labels of these pixels.

Specifically, we unprojected the 2D pixel $P_t$ to the 3D location $\bold P_t \in \mathbb{R}^3$ by following:
\begin{equation}\label{equ:project_3D}
\bold P_t=E_t^{-1}G^{-1}dP_t,
\end{equation}
where $E_t^{-1}$ is the inverse camera pose at the $t$ time step, and $d$ and $G$ are the ground truth depth and camera intrinsic matrix, respectively. 

In the next, we set all region predictions to be identical within the same local voxel $g_n$, \ie,
\begin{equation}\label{equ:refine}
\hat{R}(P^{*})=\frac{1}{|g_n|}\sum_{* \in g_n}\hat{R}(P^{*}),
\end{equation}
To this end, we obtain the spatial-temporal refined region prediction $\{\hat{R}_t(P^{*})\}_{t=1}^T$. Notably, in our panoptic segmentation formulation Eq. \ref{equ:region_classfication}, the semantics predictions $\{\hat{O}_t(\mathbb{M})\}_{t=1}^T$ of each pixel are adjusted accordingly when their region prediction is changed.

We optimize the Gaussian SLAM system by minimizing a color rendering loss $L_1\left(C_t(P),C_{GT}\right)$, a depth rendering loss $L_1(D_t(P),D_{GT})$, and panoptic prediction loss for $R_t(P)$ and $O_t(\mathbb{M})$. The objective function is as follows:
\begin{equation}\label{equ:loss_function}
\begin{aligned}
\mathbb{L} = \frac{1}{T}\sum_{t \in T}\sum_{P}\lambda_1L_1\left(C_t(P),C_{GT}\right) \\
+\lambda_2L_1(D_t(P),D_{GT}) \\ +\lambda_3CE(O_t(\mathbb{M}),\hat{O}_t(\mathbb{M})) \\
+\lambda_4DICE(R_t(P),\hat{R}_t(P^{*})) \\
+\lambda_5Sig_F(R_t(P),\hat{R}_t(P^{*})),
\end{aligned}
\end{equation}
where $\lambda_{1, ..., 5}$ are the loss weights. $L_1$ indicates the $L_1$ loss, $CE$ is the cross-entropy loss, and $DICE$ and $Sig_F$ are the dice loss and sigmoid focal loss, respectively. Following SplaTAM, we do not optimize over all previous frames, but instead select frames that are most likely to impact the newly added Gaussians. We designate every $u$-th frame as a keyframe and choose $T$ frames for optimization, including the keyframes with the greatest overlap with the current frame. Overlap is determined by analyzing the point cloud of the current frame's depth map and counting the number of points within the frustum of each keyframe.






\vspace*{-1ex}
\paragraph{SLAM System.}
The SLAM system is based on the Gaussian representation and differentiable rendering described above. Assuming we already have a map, represented by a set of 3D Gaussians, that has been created from a series of camera frames from 1 to $t$, when a new RGB-D frame $t +1$ is introduced, the SLAM system goes through the following steps: Camera Tracking, Gaussian Densification, and Spatial-Temporally Lifting. 

Firstly, the \textbf{Camera Tracking} step minimizes the image and depth reconstruction error of the RGB-D frame in relation to the camera pose parameters for $t +1$, while only evaluating errors over pixels within the visible silhouette. 

Next, the \textbf{Gaussian Densification} step adds new Gaussians to the map based on the rendered silhouette and input depth.

Finally, the \textbf{Spatial-Temporally Lifting} step updates the parameters of all the Gaussians in the scene by minimizing the RGB and depth errors over all images up to $t +1$, given the camera poses from frame 1 to $t +1$. In implementation, it optimizes a selected subset of keyframes that overlap with the most recent frame to keep the batch size manageable.

\begin{table*}[t]
  \centering
  \caption{Quantitative comparison of PanoSLAM with other semantic SLAM methods for semantic segmentation performance on Replica (mIoU(\%). We report the PQ, RQ, and SQ for each scene.}
  \label{tab:semantic_performance}
  %\vspace{-1ex}
  \scalebox{1}{
  \begin{tabular}{c |c | c |c c c c c c c c}
  \toprule
  w GT& Methods & Metrics &room0 & room1 & room2 & office0& office1& office2& office3& office4 
  \\\midrule
  \multirow{2}{*}{Yes}& NIDS-SLAM & mIoU & 82.45 & 84.08& 76.99& 85.94 &– &– &– &–
  \\ 	
  & DNS SLAM & mIoU& 88.32 &84.90& 81.20& 84.66& – &–& – &– 
  \\
  & SNI-SLAM& mIoU & 88.42 &87.43 &86.16& 87.63& 78.63 &86.49 &74.01 &80.22 
  \\\midrule
  \multirow{8}{*}{No}& \multirow{4}{*}{Baseline} & PQ & 15.2 & 13.3& 12.2 & 5.7 & 16.2 & 11.6 & 14.0 & 16.2
  \\
  &  & SQ & 27.0 & 25.3 & 23.9 & 16.6 & 30.8 & 25.2 & 24.4 & 30.8
  \\
  &  & RQ & 19.5 & 17.1 & 14.7 & 7.1 & 18.4 & 15.1 & 17.0 & 18.4 
  \\
  &  & mIoU & 49.07 & 49.80 & 39.96 & 40.06 & 67.45 & 46.95 &29.04 & 67.45
  \\\cline{2-11}
  & \multirow{4}{*}{PanoSLAM} & PQ & 19.9 & 14.1 & 18.3 & 10.6 & 16.7 & 12.8 & 14.1 & 16.3
  \\
  &  & SQ & 46.0 & 26.3 & 45.9 & 56.3 & 33.2 & 26.3 & 38.1 & 41.0
  \\
  &  & RQ & 26.6 & 18.5 & 21.9 & 14.2 & 17.6 & 16.2 & 18.3 & 13.0
  \\
  &  & mIoU & 50.32 & 50.24 & 44.14 & 42.34 & 65.2 & 47.4 & 37.40 & 68.3
  \\\bottomrule
  \end{tabular}}
  %\vspace*{-1.5ex}
\end{table*}

